3G R&D: R&D for the Next Generation of Ground-based Gravitational-wave Detectors

To deliver on the promise of next generation gravitational-wave observatories, a sustained and coordinated detector research and development program is required. This report examines in detail the wide range of nearer- and longer-term detector R&D programs needed for next generation GW detectors commensurate with the key science targets presented in "The Next Generation Global Gravitational Wave Observatory: The Science Book", including considerations of site selection and large-scale vacuum infrastructure. The report makes a series of detailed recommendations on the needed advances in detector technology and the timescales needed to achieve those advances. It also identifies areas where larger-scale globally coordinated R&D efforts will be critical to ensuring success while minimizing costs. This report is the third in a six part series of reports by the GWIC 3G Subcommittee: i) Expanding the Reach of Gravitational Wave Observatories to the Edge of the Universe, ii) The Next Generation Global Gravitational Wave Observatory: The Science Book, iii) 3G R&D: R&D for the Next Generation of Ground-based Gravitational Wave Detectors (this report), iv) Gravitational Wave Data Analysis: Computing Challenges in the 3G Era, v) Future Ground-based Gravitational-wave Observatories: Synergies with Other Scientific Communities, and vi) An Exploration of Possible Governance Models for the Future Global Gravitational-Wave Observatory Network.

==> ExecSummary.tex <==
\chapterimage{Figures1_3/summary1_3.jpg} % Chapter heading image
% Blackboard scribbles copyright Andreas Freise
\chapter{Executive Summary}
\label{sec:ExecSummary}
\pagenumbering{roman}% resets `page` counter to 1
\renewcommand{\thepage}{ES\roman{page}}
%Charge: Coordination of the Ground-based \ac{GW} Community \ac{RaD}: develop and facilitate coordination mechanisms among the current and future planned and anticipated ground-based \ac{GW} projects, including identification of common technologies and \ac{RaD} activities as well as comparison of the specific technical approaches to 3G detectors. Including identifying primary (enabling or fundamental) and secondary (or technical) technologies.
%The next generation of gravitational-wave detector will require a tight coordination of \ac{RaD} topics. 
\Ac{3G} facilities will house detectors with sensitivities at least ten times better than the \ac{2G} detectors in the whole audio band (from about 10 Hz to about 10 kHz) and more than 10000 times better at lower frequencies (below 10 Hz).
%Third generation facilities will house detectors with sensitivities at least 10 times better than \ac{2G} detectors across the audio-band (from a few Hz up to  ca.\,10\,kHz), and more than 1000 times better at the lower frequencies (below 20\,Hz). 
As with \ac{2G} facilities, the \ac{3G} infrastructures will allow detectors of successive sensitivity levels  %changed from: will enable successive generations of detectors to be installed [strictly spoken a generation is 2G, 3G, etc.]
to be installed as new technologies and techniques mature.  This report presents the main technological challenges, approaches, timelines and where possible required decision points for the realisation of a \ac{3G} network. While there are different designs and implementations for the first \ac{3G} detectors (e.g. \ac{ET}, \ac{CE}), the enabling technologies (substrates, coatings, cryogenics, suspensions, Newtonian noise cancellation, lasers and quantum enhancement) share similar challenges when viewed from the perspective of research.  Timely progress in the development of these enabling technologies requires global collaboration and coordination. To accomplish the scientific program of the 3G network, a broad coherent detector \ac{RaD} program is now required, addressing key technological challenges in the next 5-7\,years.

In our estimation, four areas in particular are of such a scale that global coordination will need to be accompanied by global \ac{RaD} funding: 

\begin{enumerate}
\item facility and vacuum infrastructure; 
\item substrates; 
\item coatings; 
\item large scale prototyping for demonstration of technology readiness. 
\end{enumerate}

\noindent Progress in areas 1, 2 and 3 will require significant involvement with industry, with some areas, e.g. coatings,  potentially requiring the \ac{GW} community to build its own fabrication facilities. Area 4 has seen recent growth, with the establishment of the 3G Pathfinder in Maastricht, but more prototyping facilities are likely to be required. Depending on \ac{RaD} progress, the first \ac{3G} detectors may adopt technologies proven in \ac{2G} facilities, scaled up to much longer baselines. Conversely, many \ac{3G} techniques may be tested or employed to improve the sensitivity of \ac{2G} detectors. 

\section{Recommendations}
\begin{itemize}
\item \textbf{Recommendation 1}:  An international \ac{3G} \ac{RaD} coordination committee should be formed, with broad and inclusive membership representing \ac{GW} groups across the world.

 A series of workshops on enabling technologies shall be held in order to stimulate exchange of ideas and allowing (if deemed useful) for coordination of the person-power intensive experimental activities.  Each of the major \ac{RaD} tasks should generate a list of  goals with quantitative metrics,  timelines and required resources.   Activities requiring global collaboration and coordination should be laid down and pathways identified.

\item \textbf{Recommendation 2}:  International consortia should be formed to work on key \ac{RaD} challenges and opportunities with industrial partners, establish a governance and organisational structure with authority and seek funding through joint proposals submitted across funding agencies.
\pagebreak
\item \textbf{Recommendation 3}: 
National funding agencies should maintain a proactive role in ensuring that the \ac{RaD} activities are well-focused and effective.  Coordination of funding plans through\ac{GWAC} would be a first step, followed by supporting the role of the international \ac{3G} \ac{RaD} coordination committee (recommendation 1) in organizing the global effort.  This is likely to require increased funding for staff and instrumentation to enable the required long-term research programs at relevant laboratories and prototype interferometers.

\item \textbf{Recommendation 4}: Existing \ac{GW} collaborations embrace \ac{3G} \ac{RaD} tasks and integrate them into their programs and deliverables, in order to ensure sufficient support for the long-term future of the field (as it has been done so successfully for \ac{2G} \ac{RaD} during the operation of the initial detectors). Over the next 5 years, mature \ac{2G} enabling technologies (e.g. 1064\,nm laser, fused silica optics, coatings) will need to be scaled up and shown ready for application in \ac{3G} facilities.



\end{itemize}

\section{}
\begin{figure}[ht]
\centering
\includegraphics*[width= \textwidth]{Figures/3G_Readiness_Levelsblue.pdf}
\caption{Approximate timelines for the required maturity levels for \ac{3G} instruments and resource levels needed from now to installation of the first phase. The estimates for the required \ac{RaD} resource level shown on the right hand side only include investment (not \ac{RaD} person costs, assumed to be supplied form the labs) and are roughly categorized into \textit{low, mid} and \textit{high}.\\
}
\label{fig:maturity}
\end{figure}

An overview of required timelines to reach installation maturity is depicted in figure \ref{fig:maturity}. The figure shows required maturity levels for the various subsystems, depending on the foreseen time of installation and anticipated lead times. Infrastructure and facilities have the longest development leadtimes and thus will have to reach maturity earliest, followed by the other subsystems in the sequence of installation. The timings for the lower \ac{ML} ML1 - ML3 (relative to the highest level ML4) depend on the duration required between the individual steps; e.g. once technical readiness is achieved for core optics it still takes a few years to demonstrate full scale prototypes and manufacture the final optics substrates through a pathfinder process. Despite considerable differences in designs for the proposed \ac{3G} observatories (\ac{ET} and \ac{CE}), large variations within the subsystems and an inevitable uncertainty in timelines, we nonetheless attempt to summarize the timelines  for each subsystem in a single bar in figure \ref{fig:maturity}.  

The resources required to reach operational readiness are roughly divided into \textit{low, mid} and \textit{high}, with indicative financial investments for \ac{RaD} for the various subsystems over the entire period from now to the start of installation. 

The highest costs for the detector elements (as distinct from the civil and vacuum construction) are expected for developing the capabilities to manufacture the main optics (presumably fused silica and silicon) and for the development of coatings and coating facilities. 
Producing ultra-pure optics substrates of approx. 200-300\,kg weight requires an international effort and tight collaboration with industry. Developing coatings of outstanding optical quality and uniformity over the whole mirror surface, combined with the required low mechanical losses at  room temperature and cryogenic temperatures is currently regarded as the biggest hurdle to overcome for building \ac{3G} gravitational wave observatories. International collaboration and building redundancy in coating capabilities is essential for success.

In particular for underground infrastructures and facilities, \ac{RaD} will incur significant costs for exploration and prototyping. Exploratory efforts have already been started at the ET candidate sites. In the construction phase, building the infrastructure and facilities will be the biggest cost items and consequently have the largest cost saving potential. \ac{RaD} efforts to minimise costs while satisfying the strict technical demands is mandatory.


%\greencomment{Stan: Good recommendations, but they would be stronger if a path to getting them accomplished was included.  For example:  instead of number4, maybe something like:
%National funding agencies should take a proactive role in ensuring that the \ac{RaD} activities are well-focused and effective.  Coordination of funding plans through GWAC would be a first step, followed by supporting the role of the international \ac{3G} \ac{RaD} coordination committee (recommendation 1) in organizing the global effort.  This is likely to require increased funding for staff and instrumentation to enable the required long-term research programs at relevant laboratories and prototype interferometers.}

% \magentacomment{Josh: Here I pasted some remarks from quantum noise that Dave suggested be moved to general considerations.} 

% \begin{itemize}
% \item National funding agencies to increase funding (staff and instrumentation) of the relevant lab activities and to enable the required long-term research programs at the relevant prototype interferometers.
% \item Existing \ac{GW} collaborations to take ownership of \ac{3G} \ac{RaD} and integrate it into their programs and deliverables, in order to ensure sufficient support for the long-term future of the field (as it has been done so successfully for \ac{2G} \ac{RaD} during the operation of the initial detectors). 
% \item Establishment of worldwide discussion and coordination forum (meeting several times a year) across all relevant collaborations, in order to stipulate exchange of ideas and allowing (if deemed useful) for a coordination of the person-power intensive experimental activities.
% \end{itemize}



==> Introduction_old.tex <==
\chapterimage{Figures1_3/Introimage.png} % Chapter heading image
%Einstein Telescope artits impression copyright Nikhef
%\section{Introduction}
\chapter{Introduction}
\label{sec:Intro}
\pagenumbering{arabic}
\setcounter{page}{1}
\vspace{-1.5cm}
In this chapter of the report we review the \ac{RaD} needed to construct and operate detectors with "third generation" or "\ac{3G}" sensitivity. 
Similar to the existing infrastructures, which initially housed the \ac{1G} \textit{\ac{LIGO}}~\cite{Abbott2009} and \textit{\ac{Virgo}}~\cite{VirgoStatus2008} detectors and now the second generation \textit{\ac{aLIGO}}~\cite{AdvancedLIGO2015} detectors, \textit{advanced Virgo}(\ac{AdVirgo}~\cite{AdvancedVirgo2015} and \textit{\ac{KAGRA}}~\cite{KAGRA2013} in a new underground infrastructure, the new \ac{3G} facilities will be designed to accommodate successive generations of detectors with increasing sensitivity as the technology evolves and new ideas emerge.
The different collaborations envisage to step-wise evolve the current \ac{aLIGO} and \ac{AdVirgo} into future enhanced versions of those detectors \ac{a+LIGO}, \ac{AdVirgo+} \cite{Zucker:LIGOAplus, Cagnoli:VirgoAplus} and later potentially into \ac{2.5G}  detectors \ac{Voyager}\cite{VoyagerDCC2018} in the same infrastructures.

 Chapter~\ref{sec:Fac_Inf} will cover the \ac{RaD} needed to select suitable sites and build such large, long-lifetime facilities in a cost efficient way. The remainder of this part will focus on the \ac{RaD} required to deliver the first detectors operational in these \ac{3G} facilities.  Currently, there are two main concepts for these detectors, \acf{ET}~\cite{ET2011}, a 10-km triangular underground detector, and \acf{CE}~\cite{CosmicExplorer2017}, a 40-km above-ground L-shaped detector. These concepts, along with the \ac{2.5G}  detector \ac{Voyager}~\cite{Voyager:Inst,VoyagerDCC2018} are highlighted in Box~\ref{Box:GWOs}.

The first instruments to be installed in the new \ac{3G} Observatories will be 10 to 20 times more sensitive than the current 
% second generation or 
\ac{2G} instruments above 100\,Hz (Fig.~\ref{fig:3GSens}).  The improvement factor exceeds 100 around 10\,Hz and thousands below 10\,Hz. Despite their differences in design, the \ac{3G} detectors \ac{ET} and \ac{CE} rely on the same 'enabling technologies' -- the main pillars on which the predictions of sensitivity are based. These technologies are used to mitigate 'fundamental noise sources' affecting the instruments, in particular: \textbf{Quantum noise} associated with the laser light fields is modified by high laser power, quantum squeezing, massive mirrors and interferometer topology; \textbf{Thermal noise} in mirror substrates, coatings and suspensions is modified by temperature and material properties (and their behaviour as a function of temperature); and \textbf{Newtonian noise} caused by the gravitational forces of moving masses (such as air, the ground, and machinery) is modified by the location of the sites and subtraction schemes. 
% quantum noise, thermal (Brownian) noise and Newtonian noise. 
%Seismic noise and residual gas noise had been listed as fundamental noises, but as they are treatable by more expensive technology we do not list them as fundamental here.

These considerations are interdependent and have implications for the detector designs. Using low temperatures to reduce Brownian noise requires a departure from the fused silica optics used in Advanced LIGO and Advanced Virgo. Sapphire and Silicon are promising low temperature materials. Silicon would require changing the operating wavelength to 1.5 -- 2\,\micro m, necessitating the development of a new suite of light sources, optical components and detectors. Considering the material properties as a function of temperature and wavelength as well as the ability to handle high optical power while minimizing noise during heat extraction from the core optics leads to four possible operating temperatures:
room temperature and the cryogenic temperatures of 123\,K, 20\,K and below 5\,K.

%%%%%%%%%%%%%%%%%%%%%%%%%
%% BEGIN DETECTORS BOX
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{DetBox}{\bf Future Gravitational Wave Observatories}
\stepcounter{boxcount}
%see definition in structure.tex
\label{Box:GWOs}
\begin{tcolorbox}[standard jigsaw,colback=amber!10!white,colframe=red!70!black,coltext=black,size=small,  title=The Einstein gravitational--wave Telescope (ET)] 
%\begin{tcolorbox}[standard jigsaw,colback=amber!10!white,colframe=red!70!black,coltext=black, size=small, title=The Einstein gravitational--wave Telescope (ET)] 
\begin{wrapfigure}{r}{0.4\linewidth}
\vspace{-10pt}
\includegraphics*[width=0.4\textwidth]{Figures/ET_Thumb.png}
\label{fig:ET_Thumb}
\vspace{-25pt}
\end{wrapfigure}
ET~\cite{ET2011} is 
%the European concept 
 a concept for a third generation gravitational-wave \emph{observatory}
 likely with a location in Europe. 
 To reduce the effects of seismic motion, the \ac{ET} concept calls for the site to be located at a depth of about 100\,m to 200\,m below ground. In its final configuration it shall be arranged as an equilateral triangle of three interlaced detectors, each consisting of two interferometers. The configuration of each detector dedicates one interferometer \ac{ET-LF}  to detecting the \textbf{L}ow \textbf{F}requency components of the gravitational-wave signal (2--40\,Hz), while the other one \ac{ET-HF}   is dedicated to the \textbf{H}igh \textbf{F}requency components, called a "xylophone" design. Each interferometer will have a dual-recycled Michelson layout with about 10\,km long \ac{FP}. In \ac{ET-LF} , which operates at cryogenic temperature, thermal, seismic, gravity gradient and radiation pressure noise sources are particularly suppressed; in \ac{ET-HF} , sensitivity at high frequencies is improved by high laser light power circulating in the \ac{FP}  cavities and the use of frequency-dependent squeezed light technologies.
\end{tcolorbox}


\begin{tcolorbox}[standard jigsaw,colframe=antiquefuchsia!80!black,colback=antiquefuchsia!20!white,opacityback=0.6,coltext=black,size=small, title=Cosmic Explorer (CE)] 
\begin{wrapfigure}{r}{0.4\linewidth}
\vspace{-10pt}
\includegraphics*[width=0.4\textwidth]{Figures/CE_Thumb.jpg}
\label{fig:CE_Thumb}
\vspace{-20pt}
\end{wrapfigure}
CE~\cite{CosmicExplorer2017} is a concept for an L-shaped above-ground observatory with 40\,km arm-length, operating a dual recycled Michelson interferometer with \ac{FP}  arm cavities, with possible site location in the US or/and in Australia. 
% CE~\cite{CosmicExplorer2017} is a US concept that envisions 40\,km long arms and new technologies to achieve a factor of 10 or more strain sensitivity improvement over the current generation of gravitational-wave detectors. 
% As with LIGO, it will employ a dual recycled Michelson interferometer with \ac{FP}  arm cavities and be implemented in stages. 
Its initial phase, called CE1, will employ scaled-up \emph{Advanced LIGO technology} including 320\,kg fused silica test masses, 1.4\,MW of optical power, and frequency-dependent squeezing. 
% Frequency-dependent squeezing will improve the quantum limited sensitivity by a factor of three. 
A major upgrade, CE2, will exploit the full potential of the new facility by using \emph{Voyager technology} such as silicon test masses and amorphous silicon coatings operating at 123\,K, with $1.5$ or $2\,\mu m$ laser light and 3\,MW of optical power in its arm cavities.

\end{tcolorbox}

%\begin{tcolorbox}[standard jigsaw,colframe=azure!70!black,colback=azure!20!white,opacityback=0.6,coltext=black, size=small, title= Voyager,sidebyside,righthand width=.3\textwidth,sidebyside gap=6mm,lower separated=false]
\begin{tcolorbox}[standard jigsaw,colframe=azure!70!black,colback=azure!20!white,opacityback=0.6,coltext=black, size=small, title=Voyager]

\begin{wrapfigure}{r}{0.4\linewidth}
\vspace{-10pt}
\includegraphics*[width=0.4\textwidth]{Figures/Voyager_Thumb.png}
\label{fig:Voyager_Thumb}
\vspace{-20pt}
\end{wrapfigure}

Voyager~\cite{Voyager:Inst,VoyagerDCC2018, VoyagerDCC2019} is the tentative concept for a new detector in the current facilities, designed to maximize the observational reach of the infrastructure and demonstrate the key technologies to be used for \ac{3G} observatories in new infrastructures.
Voyager proposes to use heavy (ca.\,200\,kg) cryogenic mirrors with improved coatings and upgraded suspensions made of ultra-pure silicon at a temperature of 123\,K in the existing vacuum envelope and a laser wavelength of $\sim1.5\,-\,2\,\mu m$. 
A further factor of 3 increase in BNS range (to 1100\,Mpc) is envisioned along with a reduction of the low frequency cutoff. %down to 10 Hz. 
In the context of this report we use the term \emph{Voyager Technology} for this type of technology irrespective of plans to implement it in any of the existing or future infrastructures.
\end{tcolorbox}

\end{DetBox}
\newpage 

%%%%%%%%%%%%%%%%%%%%%%%%%
%% END DETECTORS BOX
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{wrapfigure}{r}{0.65\textwidth}
%\begin{figure}[ht]
\centering
\includegraphics*[width= 0.64\textwidth]{Figures/noises_percentiles-Voyager.pdf}
\caption{Target sensitivity curves for \ac{3G} gravitational-wave detectors \acf{ET}~\cite{ET2011}, shown in green, and \acf{CE}~\cite{CosmicExplorer2017}, shown in pink, compared with the design sensitivity of Advanced LIGO, shown in blue. 
%and the goal sensitivity for Voyager (orange curve). 
The shades of the curves represent sensitivity to sources with differently distributed locations.}
\label{fig:3GSens}
%\end{figure}
\end{wrapfigure}

Currently, Advanced LIGO and Advanced Virgo are in their third observing run. These detectors will soon thereafter be enhanced toward LIGO A+ and AdVirgo+ operations. Following these detector upgrades by about 10 years we envision a network of new detectors, CE and ET, in new, longer-baseline \ac{3G} facilities, along with detectors that use \ac{3G} technology within \ac{2G} facilities, such as Voyager.
The key parameters of \ac{2G} and \ac{3G} instruments are summarized in Table~\ref{Tab:FutIfos}.
The \ac{3G} facilities are being designed with lifetimes up to 50 years and to be suitable for both initial instruments with sensitivities at least 10 times that of the advanced detectors and upgrades that may achieve another factor of 10.
Strategies for \ac{3G} will be modified according to observations made with current detectors, evolution in the science case, technology readiness and funds available. Nonetheless, this \ac{GWIC} \ac{3G} report represents a milestone community vision for the future of ground based gravitational wave observations. 



%Two detector epochs are envisioned 
% post advanced detector baseline sensitivities 
%to follow the advanced detectors over the next 25\,years: upgrades in existing facilities; % operating at 1\,$\mu m$ wavelength; 
%and new detectors in new, longer baseline, third generation (3G) facilities. 

%The \ac{3G} facility infrastructure can to some extent be decoupled from the initial \ac{3G} instruments. 

% There are currently two conceptual designs for such \ac{3G} facilities:  The Einstein Telescope (ET) and Cosmic Explorer (CE). A short description is given in Box \ref{Box:GWOs} and the key parameters of \ac{2G} and \ac{3G} instruments are summarized in table \ref{Tab:FutIfos}.
%The Einstein Telescope (ET) is envisaged as an underground facility capable of housing three pairs of detectors in a nested triangular vacuum envelope with three 10\,km sides. Cosmic Explorer is proposed to be a single L-shaped facility with two 40\,km arms. The most effective \ac{3G} network would incorporate a pair of widely separated Cosmic Explorers working in unison with the Einstein Telescope~\cite{Hall:2019xmm}.

Planning for the \ac{3G} detectors began more than 20 years before they are envisioned to become operative. 
This was based on experience with past and current detectors, for which there was a lead time of 15 years or more from conception to operation. 
Assuming a 2035 start date for initial \ac{3G} operations, preceded by five years of construction and five years of commissioning, it is likely that only technologies with mature \ac{RaD} in 2025 will feed into final design and engineering for the initial \ac{3G} detectors. In this document we assess the state of \ac{RaD} for \ac{3G} enabling technologies toward readiness in 2025, while also looking ahead to the \ac{RaD} that will continue as a necessary preparation for subsequent \ac{3G} upgrades. 
% Prototyping such technology may include testing performance and science capability in an existing \ac{2G} facility. The term "Voyager" is used to describe a detector in a \ac{2G} facility that would prototype \ac{CE} phase 2 technology whilst significantly improving detection range. 
Section \ref{sec:Fac_Inf} addresses requirements and design aspects of the \ac{3G} infrastructure.
In Sections \ref{sec:Core_optics} to \ref{sec:Newtonian_Noise} we consider the state of the art in enabling technologies, the \ac{RaD} needed in each area, the level of resources needed (broadly bracketed as high, medium, low), and how the \ac{RaD} should be focused in order to deliver fully tested subsystems for timely installation in new \ac{3G} facilities. 
The analysis suggests prototyping \ac{3G} technology including new test facilities and use of existing long baseline facilities. 
Sections~\ref{sec:Core_optics} and \ref{sec:Coatings} describe the closely related subjects of core optics and coatings, while Section~\ref{sec:Cryogenics} describes cryogenics, and Section~\ref{sec:Suspensions_Isolation} covers suspensions and seismic isolation systems.
A common theme among these chapters is thermal noise, described in Box~\ref{Box:Thermal}, which is the primary consideration for many choices in optics, coatings, suspensions, and operating temperature. 
Chapter~\ref{sec:Newtonian_Noise} describes Newtonian noise and its connection with facility choices and reliance on modeling and subtraction schemes. 
In addition to the fundamental noises described above, a myriad of technical noise sources and control issues can limit interferometer performance: parametric instabilities, scattered light, and noise originating from auxiliary optics and control systems. 
The current state of the art in these areas, \ac{RaD} needed, and coordination for \ac{3G} are reviewed in sections \ref{sec:Aux-optics} and \ref{sec:Sim_Controls}. 
Finally, Section~\ref{sec:Calibration} describes plans for accurately calibrating the instruments to levels that will enable the dramatic science described in the first part of this report. 

\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|p{1.6cm}|l|l|l|l|}
\hline
 % \multicolumn{8}{|c|}{Current and Future Interferometers}\\ 
 %\hline
 &aLIGO / AdV &A+/V+ &KAGRA &CE 1 &CE 2 &ET-LF &ET-HF\\
\hline
Arm Length [km] & 4 / 3 &4 / 3& 3& 40& 40& 3x10$^*$ & 3x10$^*$\\
\hline
Mirror Mass [kg]& 40 / 42& 40& 23& 320& 320& 211& 200\\
\hline
Mirror Material& silica& silica& sapphire& silica& silicon& silicon& silica\\
\hline
Mirror Temp [K]& 295& 295& 20& 295& 123& 10& 290\\
\hline
Suspension Fiber& 0.6m/0.7m& 0.6m& 0.35m& 1.2m& 1.2m& 2m& 0.6m\\
& SiO2& SiO2&Al2O3&SiO2&Si&Si&SiO2\\
\hline
Fiber Type& Fiber& Fiber& Fiber& Fiber& Ribbon& Fiber& Fiber\\
\hline
Input Power [W]& 125& 125& 70& 150& 220& 3& 500\\
\hline
Arm Power [kW]& 710 / 700& 750& 350& 1400& 2000& 18& 3000\\
\hline
Wavelength [nm]& 1064& 1064& 1064& 1064& 1550& 1550& 1064\\
\hline
\acs{NN} Suppression& 1& 1& 1& 10& 10& 1& 1\\
\hline
Beam Size [cm]& (5.5/6.2) / 6& 5.5/6.2& 3.5/3.5& 12/12& 14/14& 9/9& 12/12\\
\hline
\acs{SQZ} Factor [dB]& 0& 6& foreseen& 10& 10& 10& 10\\
\hline
Filter Cavity & none& 300& unknown& 4000& 4000& 10000& 500\\
Length [m] &&&&&&&\\
\hline
\end{tabular}
\caption{Key parameters of the current Advanced detectors, their enhancements, LIGO A+ and AdVirgo +, the two phases of Cosmic Explorer, CE1 and CE2, and the two interferometer types of Einstein Telescope. $^*$\ac{ET} will have an angle of 60$\deg$ between the detector arms}
\label{Tab:FutIfos}
\end{table}

\begin{Infobox}{\bf Thermal Noise in Gravitational Wave Detectors}
\stepcounter{boxcount}
%\label{Box:Thermal}
%\paragraph{Infobox Thermal Noise in gravitational wave detectors}
Thermal noise is one of the fundamental noise sources limiting \ac{2G} detectors over a considerable frequency range. The main contributions come from Brownian noise of the mirror suspensions, substrates and coatings and thermo-optic (thermo-elastic plus thermo-refractive) noise of substrates and coatings. The relation between the dissipation and the power spectrum (single sided) of the noise is described by Callen's Fluctuation-Dissipation Theorem~\cite{CaWe1951, Kubo:FDT, Callen:1959} and is given by:
\begin{equation}
S_x(\omega) = \frac{4\,k_B T}{\omega^2} \left| \mathrm{Re} \big[ Y(\omega) \big]\right| .
\end{equation}
\label{eq:FDT}
with \acf{k_b}, \acf{omega} , \acf{T} and \acf{Y}, defined as
\begin{equation}
Y(\omega) = i \omega\frac{X(\omega)}{F(\omega)} \, ,
\end{equation}
where \acs{DNA} and \acs{FNA} are the Fourier components of the displacement of the system and force applied leading to the displacement, respectively. The real part of the admittance is proportional to mechanical losses, hence low noise requires low mechanical losses.
Operating the mirrors and suspensions at reduced temperature reduces thermal noise since the 
%$x(\omega)$ 
\ac{DNA} scales with $\sqrt{T}$. 
%More significantly, many material properties of mirror substrates (e.g., for sapphire and silicon) and coatings (e.g., AlGaAs, AlGaP, $\alpha$-Si) scale favorably with decreasing temperature. 
%This makes the improvement in the noise potentially better than $\sqrt{T}$. Most glasses, e.g. fused silica, have increased mechanical losses at cryogenic temperatures, making them unsuited for use at cryogenic temperatures. 
More significantly, many material properties of mirror substrates and coatings depend on temperature, and hence influence the temperature dependence of thermal noise.
Fused silica, like most other glasses, has increased mechanical losses at cryogenic temperatures, making it unsuitable as substrates at cryogenic temperatures, making crystalline materials (Sapphire, Silicon) the prime candidates for low temperature operation.
Most amorphous oxide coatings show higher mechanical losses at cryogenic temperatures while the losses of crystalline or semiconductor coatings improve. The latter ones suffer from other drawbacks, e.g. optical absorption, though.
Further dependence of coating thermal noise on coating parameters is shown in Appendix~\ref{sec:Appendix_Coatings}, Figure~\ref{fig:Thermal_Noise}.
\label{Box:Thermal}
\end{Infobox}
%\end{tcolorbox}

%\begin{tcolorbox}[standard jigsaw,colframe=ocre,colback=blanchedalmond!10!white,opacityback=0.6,coltext=black,oversize,  size=small, title=Infobox~\theboxcount: Gravitational Wave Detection] 
\section{Gravitational Wave Detection Basics}
Gravitational waves induce tiny changes in separation between widely spaced “test masses”. The instrumental challenge is to measure these tiny changes. Audio band detectors use laser interferometry, where the interferometer mirrors are the test masses at the ends of long baselines whose length changes are measured. The basis of all present and next generation gravitational wave detectors is a dual recycled Fabry-Perot arm cavity Michelson interferometer as sketched in figure\,\ref{fig:ifo_layout}. 
%\begin{wrapfigure}{l}{1.1\columnwidth}
\begin{figure}[ht]
\includegraphics*[width=\textwidth]{Figures/InterferometerSchematicSubsystemColourSAS.pdf}
\caption{Schematic representation of an interferometric gravitational wave detector. Subsystems as used in this report are indicated by the colored backgrounds. The borders between subsystems are not sharply defined and somewhat arbitrary.}
\label{fig:ifo_layout}
\end{figure}
%\end{wrapfigure}

Being quadrupolar radiation, a passing \ac{GW}  alternately expands and then contracts one arm (e.g. $L_x$) of the interferometer whilst it contracts and then expands the arm perpendicular to it ($L_y$).  The effect is extremely small: expressed as a relative length change, $\delta L/L$, it is less than $10^{-22}$! The arm cavities increase the phase change imposed on the light. Interfering the single frequency light beams from the two arms at the beamsplitter (BS) cancels common noise whilst the signal adds. Extra elements (\ac{PR} and \ac{SR} mirrors, squeezing, filter cavities etc)  further increase sensitivity and optimise the response \cite{InterferometerTechniquesBond2017}.  
The core optics (test mass mirrors) are hung from sophisticated suspensions systems as indicated in figure\,\ref{fig:ifo_layout} (in the vacuum tank on the right) so that, above resonance frequencies, they are effectively free to move \cite{SuspensionsvVeggel2018}. The main optics can be cooled to cryogenic temperatures to minimise thermal noise. In addition to the  core optics there are a host of auxiliary optics to condition  and match (in angle and size) the laser beam into the interferometer  and the signal field out of the interferometer and into the photodetection system. Once technical noises, such as laser frequency and intensity noise, acoustic noise and seismic noise, have been reduced there are three basic processes limiting the interferometer sensitivity: thermal, Newtonian (gravity gradient), and quantum noise. Thermal noise \ref{Box:Thermal},\cite{ThermalNoiseHammond2014} is produced by random displacements of the mirror surfaces in response to thermally fluctuating stresses in the mirror coatings, substrates, and suspensions and it typically dominates at midband frequencies  (ca.~50-200\,Hz). . Quantum noise can be roughly divided into \ac{QRPN} and quantum phase noise or \ac{SN} \cite{QuantumNoiseBarsotti2018}. \ac{QRPN}, or quantum back-action noise arises from the random buffeting of the suspended interferometer mirrors by the quantum mechanical amplitude fluctuations of the light field being used to sense the arm-length. Shot noise results from quantum phase uncertainty: there is a limit to how well the phase difference between two light fields returning from the interferometers arms can be determined. Radiation pressure noise dominates at low frequencies (ca. 10Hz to 50\,Hz) while shot noise dominates at higher frequencies (above ca. 200\,Hz). The standard quantum limit is the noise floor for which the \ac{QRPN} and shot noise are equal at a given power level (typically around 100\,Hz). 
\Ac*{NN} arises from the direct gravitational forces exerted on the interferometer mirrors by nearby changing mass distributions primarily caused by density fluctuations of the surrounding earth due to seismic waves as well as low frequency atmospheric density changes \cite{InfrasoundNewtonianNoise2018}. 
The test masses cannot be shielded against these fluctuating forces.  In addition to the noise sources discussed above, another important issue is the suppression of instabilities that arise from photon pressure at high optical power. In reality there are a myriad of technical noise sources that need to suppressed in order to reveal the ‘fundamental limitations' (scattered light, electronic noise, various other control noises)  This is dramatically demonstrated in  figure \ref{fig:aLIGO_Noises} which shows the noise anatomy for the \acf{aLIGO} detector at Livingston, \ac{USA},  circa March 2020.  Much  of the effort and focus when commissioning  a detector is devoted to suppressing such ‘technical’  noise.
\begin{figure}
\includegraphics[width=\textwidth]{Figures/L1-READY_7A4FE0_NOISE_BUDGET-1268956818-86400.png}
% dummy picture taken from https://ldas-jobs.ligo-la.caltech.edu/~detchar/summary/day/20200302/isc/noise_budget/#gallery-1 needs to be replaced by a proper noise projection
\caption{Exemplary noise budget for \acf{aLIGO}}
\label{fig:aLIGO_Noises}
\end{figure}
%\vspace{11cm}
%\end{tcolorbox}

==> Memo.tex <==

\newpage
\section{collection of recommendation section from the various chapters}
\subsection{Facilities + Infrastructure}
collaboration with high energy particle physics community (know-how in building large vacuum
systems from accelerator facilities)

3G Infrastructure and facilities construction will start roughly 5 years before the installation of detector hardware, hence the timescales for technical readiness are shorter and more critical here.
If site preparation for the Einstein telescope is to start as early as $\sim$\,2025 the respective R\&D and detailed technical studies have to start immediately. Respective international and collaboration overarching working groups should be initiated right now.

\subsection{Core Optics}
There is not a research laboratory that is dedicated to develop and optimize the large size crystal growth with the specifications imposed by the GW detectors. This could have a severe impact on the development of 3G detectors.
\magentacomment{hal: The lead times for this R\&D are huge. Steering the direction needs decision points well ahead of time. }
timelines missing
\subsection{Coatings}
By far the most pressing timeline is for the enhanced 2G detectors. In the case of a+LIGO, allowing for a one-year pathfinder after the coating material and process are identified, the required research to identify a suitable mirror coating should be completed by May 2020. This timeline implicitly assumes that the coating will be a sputter-deposited amorphous doped oxide, perhaps deposited at an elevated temperature, a slower than conventional rate and/or with a higher than conventional annealing temperature. It is unlikely that there is time in such a schedule to identify coatings and develop the required equipment for a process with more significant deviations from current deposition methods.

In recognition of the fact that meeting the enhanced 2G detector timeline requires doing basic research on a development schedule, the efforts of the LSC community are of necessity focused on these mirrors. That said, it is also recognized that the community shouldn't put itself again in such a situation, so a portion of the current research effort is devoted to establishing approaches to mirrors for 2.5G and 3G detectors. It is difficult to set research timelines for this effort, since the funding and construction schedules for these systems are not yet established. Another open question is the deposition process that will be required for the 2.5G and 3G mirrors; the further that process is from conventional IBS, the longer it is likely to take to develop suitable tooling. It seems that in any plausible scenario at least five years are available for research into the best approach to mirrors meeting 2.5G requirements. Results for these 2.5G mirrors will, in turn, inform choices with respect to 3G mirrors. It is therefore too soon to argue for a large investment in scaling deposition tools alternative to elevated-temperature IBS for 2.5G and 3G mirrors. That said, as the funding trajectories and interferometer architectures become better defined, it will be important to regularly re-evaluate the current understanding of potential mirror technologies, and make critical decisions, especially with respect to deposition tools with long development times and requiring major financial investments.

\subsubsection{Recommendations}

\noindent The additional funding provided by the CCR for U.S. efforts in coating research, combined with the previously existing NSF support, leave these efforts with reasonably adequate funding in the near future. It would be helpful to add another deposition group to the effort, as there is currently more capacity for characterization of properties (other than cryogenic mechanical losses) than for synthesis. It is also important that the LIGO Lab continue with at least its current effort level, as their contribution to high-throughput mechanical loss characterization, optical scatter and homogeneity measurements, and their overall coordination of sample fabrication, distribution, and characterization is important to the LSC efforts.

In GEO, there is growing capacity for depositing coatings at Strathclyde, UWS and Hamburg. These coatings can be produced at a rate faster than it is possible to characterize their properties at cryogenic temperatures, and thus more resources devoted to such characterization are desirable. Currently, a novel type of ion-beam sputtering is being developed and tested at Strathclyde. While this is a promising research route, there are also plans to set up a large chamber with an industry ion source which should be capable of producing large and uniform enough coatings. This is an important priority in gaining access to more coating facilities which are suitable for the deposition of large, high-quality coatings. Initiating studies of GaP/AlGaP crystalline coatings, using hardware now installed in an MBE chamber at Gas Sensing Solutions Ltd, is also planned. This is an important parallel research direction to the development of amorphous coatings.

In VIRGO, the activities are progressing at the pace compatible with the funding available from other projects. \magentacomment{Josh: I do not understand what the previous sentence intends to say.} LMA and University of Sannio are able to provide high quality coatings at a rate higher than the existing characterization capability in VCR\&D. The project ViSIONs takes care of only one specific aspect of the research, that is the impact and the understanding of deposition parameters on the coatings properties.

At present, there is only one institution, LMA, capable of depositing coatings of a size and quality suitable for gravitational wave interferometers. LMA will continue to be supported as a research and coating facility for future GW detectors by the French CNRS through EGO, while support for another institution, CSIRO in Australia, which was able to provide similar coating quality, was discontinued some time ago. It seems prudent to restart this program to create redundancy through a second source of high quality coatings and to have another significant contributor to ongoing research efforts. Within these activities, the products of other commercial vendors can also be characterized. 
Continued and deeper coordination among all GW collaborations will be critically important in developing coatings with the requisite 3G performance.

\subsubsection{Roadmap}
Since the development of low-thermal-noise coatings is in the stage of research rather than development, even for 2.5G detectors, a conventional roadmap would not seem the best model for describing the path towards identifying suitable mirror designs and fabricating corresponding full-scale mirrors for 3G detectors. Noting that the architectures and operating parameters for 3G detectors remain in flux, that the results for mirrors developed for 2.5G detectors will have a strong, perhaps determinative, influence on the designs for 3G mirrors, and that the funding and thus construction schedules for 3G detectors are not yet clear, it is best to estimate schedule implications in terms of times before installation. Here we discuss aspects that will drive the necessary decisions, and estimate the time prior to anticipated installation in 3G detectors that various steps must be completed. 
The currently plausible approaches to 3G mirrors fall into three broad categories which have different cost and schedule drivers: amorphous coatings deposited by methods similar to conventional ion-beam sputtering (IBS), amorphous coatings deposited by alternative means, e.g. chemical-vapor deposition (CVD), and crystalline coatings. 
Amorphous coatings deposited by IBS methods: IBS is currently the only mature technology for depositing mirrors suitable for GW interferometers (GWI); the challenge is identifying suitable combination of materials and deposition conditions (rate, ion energy, substrate temperature, …) to meet mechanical loss and optical specs. Time required for this step is open-ended; a solution might be found next month, or might not exist at all. Once materials and conditions are determined, the time required to reach the production stage depends on the deviation from current IBS practice: for room-temperature deposition at conventional rates, perhaps a 1-2 year pathfinder would be adequate. For more extreme conditions of elevated substrate temperature, low rate, high ion energy, ion-beam assist, nanolayers, microwave annealing, … perhaps 3-5 years and USD 3-5M for developing suitable equipment and the pathfinder process might be required. Multi-material coatings would lie between these extremes of time and equipment cost. 
Amorphous coatings deposited by methods other than IBS: If research shows the optimum  deposition method is other than IBS, for example chemical vapor deposition (CVD) of a-Si/SiNx mirrors, in addition to open-ended research time similar to the IBS case, adequate time would be required to develop deposition tools and a scaled up process suited to GWI requirements. While CVD tools are widely used in the semiconductor industry, adaptation to GWI mirror requirements would be a significant effort. Instrumentation development and the more complex pathfinder process might require  USD 25-30M and perhaps 10 years. These figures are order of magnitude estimates that likely could be tightened up through discussions with equipment vendors. 
Crystalline coatings: For AlGaAs crystalline mirrors, the materials research and modeling phase for small scale (ca. 6 inch) coatings could be completed in perhaps three years. If these results showed GWI level performance, the time and financial costs for substrate and tool development and the more complex pathfinder process to scale to GWI size optics might be USD 25M and 10 years. 


\subsection{Cryogenic}
\subsubsection{Pathways, required facilities and collaborations}
%
For each operating temperature (below 20\,K, 123\,K)


\begin{enumerate}
\item demonstrate reliable and timely  heat extraction and required final temperature stability (varies depending on goal material parameters).
\item demonstrate integration with SIS   (Nb: requirements differ for CE and ET).
\item demonstrate integration with other subsystems.  eg auxiliary optics  for  wave front control .
\item system integration and performance  testing on large scale prototypes/detectors.
\end{enumerate}

A key element of any cryogenic implementation is a refrigerator that is as quiet and vibration free as possible. R\&D devoted to design and construct silent refrigerator machine is required.  Several ideas have been proposed, for example the use of PT cryocoolers with symmetric cold heads.  Collaboration with cryogenics industry and the accelerator community is strongly recommended. 

For sapphire core optics at 20\,K:   Items 1 and 3 have been/will be demonstrated using KAGRA.  As the current sensitivity goal of KAGRA is modest at low frequencies, it is not clear how well KAGRA performance will inform item 2 and 4.  May occur with KAGRA upgrade.

Silicon core optics at 18\,K, 123\,K : Items 1-3:  a number of facilities are planned or under construction.  Existing facilities  at Stanford, Caltech and Gingin are currently being reconfigured. A  new facility at Maastricht in Europe has been designed to investigate  both 123K and  below 20\,K. Much of the required technology for cryogenic operation is also needed in the near term for  exploration of  the material properties of mirrors, coatings, etc.  \textit{Tight coordination is needed between these groups to  ensure optimum focus and timely progress.}

Ultimately full system integration tests (Item 4) need to be done on large, sensitive, prototypes, demonstrating sustained high performance.  The prototypes need to be large enough to allow reliable scaling to full size 3G systems.  \textit{\textbf{This is a major undertaking and global collaboration is needed to resource, develop and manage these prototypes}}.  These could be new facilities, or,  potentially, an existing 4\,km facility(ies) could be re-purposed.  This would not only demonstrate technical readiness but would produce detector(s) with a significantly extended range.  This is effectively the Voyager concept.

Cooperation with high-energy particle physics, where comparable requirements are addressed, could create valuable synergies. Furthermore, the use of cryogenics in the electronics and the magnetic actuators\cite{cryo:OSEM} has the potential to be of great benefit. These techniques should be explored in parallel with the more fundamental cryogenic interferometry.

\subsubsection{Roadmap}

\textit{Sapphire at 20\,K}


\begin{itemize}
\item  2019-2026  	Use KAGRA to diagnose  feasibility and performance.
\item  2027  		First Cryogenic downselect.  
\item  2028-2032  		If GO:  final design and fabrication.
\end{itemize}



\textit{Silicon at 	123\,K}
•  \begin{itemize}
\item 2019-2025  	R\&D in university labs on 1. and 3.
\item 2022-2028	Integration testing with SIS and other subsystems  (item 2).
\item 2028……  	Cryogenic downselect
\item 2029-2033	Large  Phase noise prototype
\item 2034-2039		If GO:  final design and fabrication.
\end{itemize}



\textit{Silicon at 	18\,K}
\begin{itemize}
\item SAME CYCLE AS SILICON AT 123\,K.
\end{itemize}

Note that it is feasible that both Silicon 123\,K and Silicon 18\,K cryogenic subsystems will be deployed at different 3G facilities.  Depending on facility finding and  technology readiness, it is  feasible, perhaps even likely,  that 3G facilities will initially operate room temperature detectors whilst cryogenic development continues.

\subsection{Newtonian Noise}
The main facilities of NN R\&D are the natural environments of 3G detector candidate sites. In addition, since we have very little experience in observing and modelling underground seismic and sound fields, underground studies done anywhere can provide important information. There are significant differences between sites in terms of sources of environmental disturbance, local geology and topography, so transferring results from one site to another should be done with caution.

Finite-element simulations of environmental fields and algorithms for the optimization of array configurations for noise cancellation are computationally expensive. Significant computing time on clusters will be required. 

Collaboration between groups is strongly recommended with respect to site characterization. It requires substantial expertise to set up robust, high-quality environmental measurements, to understand, which properties of environmental fields need to be understood, and how to analyze environmental data. Collaboration is also encouraged between groups working on numerical simulations to share generic knowledge, e.g., of how to assess accuracy of numerical simulations, e.g., by comparing simulations using different software, or by running simple simulations that allow comparison with analytic models.
\subsection{Light Sources}
Like in the past a strong collaboration between a group within the GWD community and a laser research lab or industry is required (like e.g.  AEI/LZH, Artemis/Alphanov, ICRR/Mitsubishi) to design and build suitable HPLs at the different wavelengths. As the different wavelengths need different solutions a loose collaboration between the respective wavelength groups would be advantageous. It would be desirable to have at least two collaborations to work on laboratory prototype solutions for each wavelength to explore different concepts and alternative technical solutions. These groups should have a strong connection with regular meetings to exchange results and ideas. This approach would possibly avoid a single supplier problem.
No particular collaborations are required for the squeezing research. The normal exchange of concepts and results at collaboration meetings and conferences seems sufficient. 

\subsubsection{Road map}
\subsection*{HPL 1064\,nm}
\begin{itemize}
	\item 2019 - 2020 : continue development and reliability studies of 2G PSL systems at the 250\, W level and perform coherent combination demonstration experiments at high powers
	\item 2021 - 2024 : engineering prototype (see section \ref{sec:pathway}) 500\,W HPL and conceptual test of stabilization and spatial filter solutions
	\item 2024 - ... : final design and fabrication of HPL with the initial 3G requirements within specific 3G GWD project, in parallel R\&D on path toward the final 3G requirements 
\end{itemize} 


\subsection*{HPL ${\bf 1.5 - 2.1 \, {\bf \mu m}}$}
\begin{itemize}
	\item 2019 - 2021 : identify concepts for a 1\,kW HPL that fulfills the stringent 3G GWD HPL requirements (most likely several coherently combined stages)
	\item 2022 - 2024 : 1\,kW HPL functional prototype phase (see section \ref{sec:pathway})
	\item 2024 - 2028 : 1\,kW HPL engineering prototype phase (see section \ref{sec:pathway})
	\item 2028 - ... : final design and fabrication of HPL with the initial 3G requirements within specific 3G GWD project, in parallel R\&D on path toward the final 3G requirements
\end{itemize} 


\subsection*{squeezed light sources for 3G GWDs}
\begin{itemize}
	\item 2019 - 2026 : continue laboratory based R\&D on squeezed light sources at all wavelength, potentially involve industrial partners to design and fabricate low loss optical components
	\item 2026 - ... : final design and fabrication within specific 3G GWD project
\end{itemize}
\subsection{Quantum enhancements}
A significant R\&D effort is required to make an informed selection of the optimal quantum noise reduction strategies for 3G detectors and to enable their risk free application to maximise the science return of 3G observatories. Additionally, we recommend the development of unified classification scheme of QND techniques and common approach to analysing and comparing their performances.  

\magentacomment{hal: timelines???}

\subsection{Suspensions and Seismic Isolation Systems}

It is important to note that it has typically taken 10-15 years to take suspension and seismic isolation hardware from prototype designs to interferometer installation. Thus prototypes for 3G suspension and isolation systems are an essential step to take in the near future. These can start with small scale (bench top) prototypes. However full-scale test facilities will also be needed. 2G facilities such as LASTI (MIT), the 40m detector (Caltech), Gingin (Western Australia)
% (others e.g. in Virgo and Kagra) 
or upgrades to those can be used as test beds for 3G ideas. There is also a pressing need for new prototypes, especially for cryogenic testing, such as ``ET pathfinder."

\subsubsection{Type of collaboration required and suggested mechanisms}

Several small-scale collaborations across detector groups in different countries already exist and we expect these to continue.  Ideas and results can be shared and discussed at existing meetings such as GWADW or other meetings such as ET workshops. No other large collaborations are currently envisioned.

\magentacomment{hal: timelines???}
\subsection{Auxiliary Optics}

\paragraph{\bf Light sources} Many of the auxiliary optics subsystems will be strongly impacted by the choice of laser wavelength. Beyond this, the input optics has a direct interface with the light source, and so information exchange between groups performing R\&D in these two areas will be critical.
\subsubsection{\bf Quantum noise} The output optics subsystem will be closely linked to the quantum noise working groups as squeezing is foreseen in all future detectors. Close collaboration between these groups will therefore be beneficial.

\magentacomment{hal: timelines???}
\subsection{Simulation and Controls}
\subsubsection{roadmap Sim}
Simulation tools are strongly defined through the context in which they are used. Many of the priorities for the research and development directly translate into a priority task for modelling work or a required effort in developing new capabilities for simulation tools. In particular the progress in modelling tools or modelling itself is not limited by development of technologies or methods, but by the available person power.

%%% -------------------------------------------------------------------------
\subsubsection{Recommendations Sim}
To address the above challenges, the current portfolio of software tools must be updated, either by extending the existing software or by providing new dedicated tools. The detailed list of code changes or required features goes beyond the scope of this document. The following are recommendations for the higher-level actions to support an effective and open environment for this effort.

\noindent{\textbf{Additional software}}
Most of the required modelling tasks can be performed by extending and updating the available tools, some of which is already well underway. However some missing functionality might be better achieved by developing new software. Needed packages include an easy to use and flexible time-domain simulation, a 3D beam tracing software dedicated to ground based detectors and a comprehensive modelling software for various suspension systems capable of computing the thermal noise of all elements. In addition, commercial tools should be reviewed to understand when these are superior to custom made tools, for example, for more common optics tasks such as modelling stray light.

\noindent{\textbf{Resources}}
We encourage institutions to increase support for the development and use of simulation tools over the next 5 years, a crucial time for the design of 3G instruments, and for upgrades to current detectors.
%, while the commissioning of detectors will push the limits of current technology. 
Experience has shown that
individual post-docs and PhD students can provide effective tools that are quickly adopted and used by a wide community. However, those tools often come only with rudimentary or outdated documentation and code reviews or formal testing of simulation results are not common practice. We recommend additional, dedicated post-doc support in this area to mitigate this.

\noindent{\textbf{Collaboration and coordination}}
Coordination between research groups and projects is important in three ways:
code development is often done by few individuals in each project who will benefit from having a forum to discuss priorities as well as technical challenges. The same is true for the collaboration between people
%undertaking the code development and those 
doing modelling, often 
%Modelling tasks (design or commissioning) are often 
investigating a new or not-understood behaviour;
collaboration with other scientists investigating similar or related aspects has been shown to greatly reduce the time to reaching a conclusion. We recommend to continue (or establish) working groups dedicated to the interferometer modelling within projects and 
%for these working groups 
to organize workshops/meetings adjacent to international meetings.

\noindent{\textbf{Software and code distribution}}
Accessibility of the software, and ideally the source code, should be improved. Each software tool should have: a) an active maintainer who is responsible for the current code base and who can be identified and reached by any users of the software, b) a single, discoverable web page hosting the master version of the tool or code under a clear and permissible software license, c) documentation about the implemented models and their limitations, including descriptions of mathematical algorithms, or parameter sets used and d) training material, such as a set of examples and tutorials for new users, especially graduate students. Where possible (without breaking existing compatibility) the adoption of common  input and output formats, for example, for files storing interferometer parameters  should be encouraged.

The effectiveness of specific tools is often not defined by the a single feature but by a network effect based on many factors. Any tool benefits greatly from a large user base, for example, through receiving bug reports and the availability and diversity of examples as well as experts on how to use the specific tool. And the impact of a modelling tool is improved significantly by a strong track record and trust by the wider community. We recommend that software maintainers adopts the aim of making the software as accessible as possible without compromising its core functionality. %Similarly we recommend that groups distributing software make an effort in providing training material or training opportunities for new users. The quality and effectiveness of simulation tools can be greatly enhanced by a large and informed active user base.

Those software tools that aim at providing standard results for the wider community must also provide the official data sets or model files, such as, for example default LIGO models for \textsc{Finesse}. The GWINC software package should provide standard noise budgets for all envisaged detectors and the
collaborations should establish a mechanism to review its noise models by the international community.

\noindent{\textbf{Source code maintenance}}
Some important simulation tools date back to their original development in the 80s and 90s. Given the rapid development of computing and computer languages, it could be beneficial to re-implement these in modern frameworks. At the same time the experience and knowledge acquired with the originals should not be lost in the process. A careful development process and code design that finds a balance between modern technology and backwards compatibility
is recommended. Some codes, such as \textsc{Finesse} and GWINC are currently undergoing such a process. Other software should be reviewed for similar updates.

\subsubsection{Roadmap Controls}
Similarly to simulations, progress in the development of the required controls is not defined by future technical breakthroughs in the topic itself. Instead we can adapt techniques that have been developed in other areas, such as modern control techniques. Simulation tools can play a crucial role for designing control techniques and they should be further developed or extended for this purpose.
More advanced techniques, such as adaptive control or machine learning, might need different and more powerful hardware to run, for example dedicated FPGAs or GPUs. 
It is important to advance the control design compared to other subsystems, so that controls can inform the overall system design, which allows to avoid mistakes that make the control harder or impossible. Prototype interferometers have to be used for the experimental validation of control schemes when these incorporate a more fundamental change, whereas other techniques might be implemented and tested directly in current detectors.


\subsubsection{Recommendations Controls}
Control noise, or cross-coupling of fundamental noise through control channels, has historically limited GW detectors, especially at the low-frequency end of the measurement band. The requirements of 3G detectors will pose a great challenge to control systems. Control schemes should be developed and tested early as an integral part of detector designs. Synergies with commissioning and detector upgrades should be sought out. At the same time, care should be taken that sufficient theoretical work and tests at prototype interferometers are performed for new control designs that cannot be tested with current detectors.

\subsection{Calibration}

Requirements on the absolute and relative calibration for third-generation detectors are not yet fully known, and dedicated modeling efforts are needed to understand the constraints set by various 3G scientific objectives. 3G detectors will likely require well sub-percent amplitude calibration, potentially necessitating R\&D to improve the capabilities of the current calibration apparatuses; such R\&D is already underway and cooperation activities between the different GW collaborations are considered to be at an adequate and sufficient level. 

%\input{ExecSummary.tex}

==> Participants.tex <==
\chapterimage{Figures/Test.jpg} % Chapter heading image
%\section{Introduction}
\chapter{Participants / Authors}
\label{sec:Participants}


McClelland, David, \texttt{david.mcclelland@anu.edu.au}
\\
L\"uck, Harald,   \texttt{harald.lueck@aei.mpg.de} 
%Inst. f. Gravitationsphysik, Leibniz Universitaet Hannover and Max-Planck Institut f. Gravitationsphysik, Hannover, Germany; 
\\
v.d. Brand, Jo, \texttt{jo@nikhef.nl} 
\\
Adhikari, Rana, \texttt{rana@caltech.edu}
\\
Billingsley, Garilynn, \texttt{billingsley\_g@ligo.caltech.edu}
\\
Cagnoli, Gianpietro, \texttt{gianpietro.cagnoli@univ-lyon1.fr}
\\
Evans, Matthew, \texttt{mevans@ligo.mit.edu}
\\
Fejer, Martin, \texttt{fejer@stanford.edu}
\\
Fidecaro, Francesco, \texttt{francesco.fidecaro@unipi.it}
\\
Freise, Andreas, \texttt{adf@star.sr.bham.ac.uk}
\\
Fulda, Paul, \texttt{pfulda@phys.ufl.edu}
\\
Gemme, Gianluca, \texttt{gianluca.gemme@ge.infn.it}
\\
Genin, Eric, \texttt{eric.genin@ego-gw.it}
\\
Gonzalez, Gabriela, \texttt{gonzalez@lsu.edu}
\\
Harms, Jan, \texttt{jan.harms@gssi.it}
\\
Hild, Stefan, \texttt{stefan.hild@ligo.org}
\\
Losurdo, Giovanni, \texttt{giovanni.losurdo@pi.infn.it}
\\
Lough, James, \texttt{James.Lough@aei.mpg.de}
\\
Martin, Iain, \texttt{iain.martin@glasgow.ac.uk}
\\
Massaki, Ando,  \texttt{ando@phys.s.u-tokyo.ac.jp}
\\
Prabhakar, Anil, \texttt{anilpr@ee.iitm.ac.in}
\\
Reid, Stuart, \texttt{Stuart.Reid@strath.ac.uk}
\\
Ricci, Fulvio, \texttt{fulvio.ricci@roma1.infn.it}
\\
Robertson, Norna, \texttt{nroberts@ligo.caltech.edu}
\\
Willke, Benno, \texttt{Benno.willke@aei.mpg.de}
\\
Yamamoto, Kazuhiro \texttt{yamak@icrr.u-tokyo.ac.jp}



==> WavelengthChoice.tex <==
\chapterimage{Figures/Test.jpg} % Chapter heading image
\chapter{Wavelength Choice}
%\section{Wavelength Choice}
\label{sec:wavelength}
How to choose the laser wavelength?
\magentacomment{hal: Do we need this section or shall we include it somewhere else?}

==> authors.tex <==
\newcommand*{\email}[1]{\normalsize , \href{mailto:#1}{#1}}
\newcommand*{\noemail}[1]{}

%*************
% for author numbers to be automated, gets tricky if there are authors from the same institutions
%\newcounter{authnum}[section]
%\setcounter{authnum}{1}
% \theauthnum %usage of the new counter
% \stepcounter{authnum} %increase counter by one



\author[1]{McClelland, David E.\email{david.mcclelland@anu.edu.au}}\par
\affil[1]{Centre for  Gravitational Astrophysics \& the ARC Centre of Excellence for Gravitational wave Discovery (OzGrav), The Australian National University,  Canberra, 2601,  Australia} 

\author[2]{L\"uck, Harald\email{harald.lueck@aei.mpg.de}} \par
\affil[2]{Max-Planck Institut for gravitational physics \& Institut f\"ur Gravitationsphysik der Leibniz Universit\"at Hannover, Callinstr. 38, 30167 Hannover, Germany} 
\author[3]{Bertolini, Alessandro\email{alberto@nikhef.nl}}  \par
\affil[3]{Alessandro Bertolini, Nikhef, Science Park 105, 1098XG Amsterdam, The Netherlands}
\author[3]{van den Brand, Jo\email{jo@nikhef.nl}} 
\author[4]{Adhikari, Rana\noemail{rana@caltech.edu}} \par
\author[5]{Billingsley, GariLynn\email{billingsley\_g@ligo.caltech.edu}} \par
\affil[5]{California Institute of Technology, Pasadena, California 91126, USA}
\author[6]{Cagnoli, Gianpietro\email{gianpietro.cagnoli@univ-lyon1.fr}} \par
\affil[6]{Univ Lyon, Univ Claude Bernard Lyon 1, CNRS, Institut Lumi\`ere Mati\`ere, F-69622, VILLEURBANNE, France}
\author[7]{Danilishin, Stefan\email{s.danilishin@nikhef.nl}} \par
\affil[7]{Department of Gravitational Waves and Fundamental Physics, Maastricht University, 6200 MD Maastricht, The Netherlands, and Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands}
\author[8]{Evans, Matthew\email{m3v4n5@mit.edu}} \par
\affil[8]{Department of Physics, Massachusetts Institute of Technology, 77 Mass Ave. Cambridge Massachusetts USA}\par
\author[9]{Fejer, Martin\email{fejer@stanford.edu}} \par
\author[10]{Fidecaro, Francesco\email{francesco.fidecaro@unipi.it}} \par
\affil[10]{University of Pisa and INFN, Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy}
\author[11]{Freise, Andreas\email{a.freise@nikhef.nl}} \par
\affil[11]{Department of Physics and Astronomy, VU Amsterdam, De Boelelaan 1081, 1081, HV, Amsterdam, The Netherlands, and Nikhef, Science Park 105, 1098, XG Amsterdam, The Netherlands}
\author[12]{Fulda, Paul\email{paulfulda@ufl.edu}} \par
\author[13]{Gemme, Gianluca\email{gianluca.gemme@ge.infn.it}} \par
\affil[13]{INFN, Sezione di Genova, I-16146 Genova, Italy}
\author[14]{Genin, Eric\email{eric.f.genin@gmail.com}} \par
\affil[14]{European Gravitational Observatory, via E. Amaldi,  I-56021 Cascina, Italy}
\author[15]{Gonzalez, Gabriela\email{gonzalez@lsu.edu}} \par
\affil[15]{Department of Physics and Astronomy, Louisiana State University, 2020 Nicholson, Baton Rouge, LA, USA} \par
\author[16]{Hammond, Giles\email{giles.hammond@glasgow.ac.uk}} \par
\affil[16]{SUPA, Institute for Gravitational Research, School of Physics and Astronomy, University of Glasgow, Glasgow, G12 8QQ, UK}
\author[17]{Harms, Jan\email{jan.harms@gssi.it}} \par
\affil[17]{Gran Sasso Science Institute (GSSI), I-67100 L'Aquila, Italy \&
INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi, Italy}
\author[7]{Hild, Stefan\email{stefan.hild@maastrichtuniversity.nl}} \par
%\author[3]{Li, Ju\email{ li.ju@uwa.edu.au}}  \par
\author[14]{Losurdo, Giovanni\email{giovanni.losurdo@pi.infn.it}} \par
\author[2]{Lough, James\email{James.Lough@aei.mpg.de}} \par
\author[18]{Majorana, Ettore\email{Ettore.Majorana@roma1.infn.it}} 
\affil[18]{Ettore MAJORANA, Dipartimento di Fisica, Sapienza Università di Roma, P.le A. Moro 2, 00185 Roma - Italy}\par
\author[19]{Martin, Iain \email{iain.martin@glasgow.ac.uk}} \par
\affil[19]{SUPA, Institute for Gravitational Research, School of Physics and Astronomy, University of Glasgow, UK.}
\author[20]{Massaki, Ando\email{ando@phys.s.u-tokyo.ac.jp}} \par
\affil[20]{Department of Physics, The University of Tokyo, Hongo 7-3-1,Tokyo 113-0033, Japan}
\author[21]{Prabhakar, Anil\email{anilpr@iitm.ac.in}} \par
\affil[21]{Department of Electrical Engineering, IIT Madras, Chennai 600036, India.}
\author[22]{Reid, Stuart \email{Stuart.Reid@strath.ac.uk}} \par
\affil[22]{SUPA, Department of Biomedical Engineering, University of Strathclyde, UK.}
\author[15]{Ricci, Fulvio\email{fulvio.ricci@roma1.infn.it}} \par 
%\affil[23]{Department of Physics,{\it Sapienza} university of Rome \& INFN, sezione di Roma, Piazz. A. Moro 5, I-00185 Roma, Italy}
\author[24]{Robertson, Norna\email{nroberts@ligo.caltech.edu}} \par
\affil[24]{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA \&
SUPA, University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\author[25]{Smith, Joshua\email{josmith@fullerton.edu}} \par
\affil[25]{Nicholas and Lee Begovich Center for Gravitational-Wave Physics and Astronomy, California State University, Fullerton, Fullerton, California 92831, USA}
%\author[3]{Suzuki, Yoichiro\email{suzukit@icrr.u-tokyo.ac.jp}} \par
\author[26]{Vocca, Helios\email{helios.vocca@unipg.it}} \par
\affil[26]{University of Perugia, via A. Pascoli, I-06123 Perugia, Italy and
INFN, sezione di Perugia, I-06123 Perugia, Italy}
\author[2]{Willke, Benno\email{Benno.willke@aei.mpg.de}} \par
\author[27]{Venkateswara, Krishna\email{kvenk@uw.edu}} \par
\affil[27]{University of Washington, Seattle, WA 98195, USA}
\author[1]{Ward, Robert L.\email{robert.ward@anu.edu.au}}\par
\author[28]{Yamamoto, Kazuhiro \email{yamamoto@sci.u-toyama.ac.jp}} \par
\affil[28]{Department of Physics, University of Toyama, 3190 Gofuku, Toyama 930-8555, Japan}

==> defs.tex <==
\def\newacronym#1#2#3{\gdef#1{#3 (#2)\gdef#1{#2}}}

%%%%%%%% common commands
\def\gw#1{gravitational-wave#1 (GW#1)\gdef\gw{GW}}
\def\grb#1{gamma ray burst#1 (GRB#1)\gdef\grb{GRB}}

\newacronym{\NR}{NR}{Numerical Relativity}
\newacronym{\GR}{GR}{General Relativity}


\def\th{\textrm{\mbox{\tiny{th}}}}
\def\Tobs{T_{\textrm{\mbox{\tiny{obs}}}}}
\def\Tcoh{T_{\textrm{\mbox{\tiny{coh}}}}}
\def\nd{{\mathbf{n}}_d}
\def\SSB{\textrm{\mbox{\tiny{ssb}}}}
\def\ns{\textrm{\mbox{\tiny{NS}}}}
\def\min{\textrm{\mbox{\tiny{min}}}}
\def\max{\textrm{\mbox{\tiny{max}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\N{\textit{\mbox{\tiny{N}}}}
\def \calf {\cal F}
\def\etal{{\it et al.}}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\un}[1]{\mathrm{\,#1}}
\newcommand{\ee}[1]{\!\times\!10^{#1}}
\newcommand{\Qhat}{{\widehat{Q}}}
\newcommand{\What}{{\widehat{W}}}
\newcommand{\rd}{\,{\rm d}}
\newcommand{\avec}{\mbox{\boldmath$a$}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\mtot}{\mathrm{M}_{\mathrm{T}}}
\newcommand{\msun}{\mathrm{M}_{\odot}}
\newcommand{\Msun}{\mathrm{M}_{\odot}}
\newcommand{\Mtot}{\mathrm{M}_{T}}

\newcommand{\np}{\vspace{0.2cm}\noindent}


\def\th{\textrm{\mbox{\tiny{th}}}}
\def\Tobs{T_{\textrm{\mbox{\tiny{obs}}}}}
\def\Tcoh{T_{\textrm{\mbox{\tiny{coh}}}}}
\def\nd{{\mathbf{n}}_d}
\def\SSB{\textrm{\mbox{\tiny{ssb}}}}
\def\ns{\textrm{\mbox{\tiny{NS}}}}
\def\min{\textrm{\mbox{\tiny{min}}}}
\def\max{\textrm{\mbox{\tiny{max}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\N{\textit{\mbox{\tiny{N}}}}
\def \calf {\cal F}
\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\vs{{\it vs.}}
\def\fstat{$\calf$-statistic}
\newcommand{\G}{\mathcal{G}}

% ---- Burst-specific commands.
\newcommand{\cwb}{\textsc{cwb2g}}
\newcommand{\stamp}{\textsc{stamp}}
\newcommand{\stampas}{\textsc{stamp-as}}
\newcommand{\ep}{\textsc{excesspower}}
\newcommand{\xp}{\textsc{x-pipeline}}
\newcommand{\lib}{\textsc{lib}}
\newcommand{\bw}{\textsc{bayeswave}}
\newcommand{\kw}{\textsc{kleine-welle}}
\newcommand{\om}{\textsc{omicron}}  
\newcommand{\bwg}{Burst Group}

% CBC group definitions
\newcommand{\MBTA}{\textsc{\ac{MBTA}}\xspace}
\newcommand{\LLOID}{\ac{LLOID}\xspace}
\newcommand{\GSTLALCBC}{\textsc{Gstlal-CBC}\xspace}
\newcommand{\ahope}{\textsc{aHope}\xspace}
\newcommand{\bayestar}{\textsc{Bayestar}\xspace}
\newcommand{\lalinference}{\textsc{LALInference}\xspace}
\newcommand{\pycbc}{\textsc{pyCBC}\xspace}
\acrodef{CBC}{Compact Binary Coalescence}
\acrodef{GW}{gravitational-wave}
\acrodef{BNS}{binary neutron star}
\acrodef{NS}{neutron star}
\acrodef{NSBH}{neutron star black hole binary}
\newacronym{\BBH}{BBH}{black hole binary}
\acrodef{EM}{electromagnetic}
\acrodef{EOS}{equation of state}
\acrodef{GRB}{gamma-ray burst}
\acrodef{LLOID}{Low-Latency Online Inspiral Detector}
\acrodef{MBTA}{Multi-Band Template Analysis}

% Computing definitions
\newcommand\ligocomputing{LIGO Computing}
\newcommand\tieronesites{Tier-1-Observatories}
\newcommand\tieronecit{Tier-1-Caltech}
\newcommand\tiertwoshared{Tier-2-Shared}
\newcommand\tiertwoother{Tier-2-Other}
\newcommand\ldg{LDG}
\acrodef{LSC}{LIGO Scientific Collaboration}
\acrodef{LDR}{LIGO Data Replicator}
\acrodef{LDG}{LIGO Data Grid}
\acrodef{iLIGO}{initial LIGO}
\acrodef{aLIGO}{advanced LIGO}
\newacronym{\aligo}{aLIGO}{Advanced LIGO}


% from the Observing Scenario Document
\def\aLIGOEarly{60}
\def\aLIGOEarlyU{40 -- 80}
\def\aLIGOMid{100}
\def\aLIGOMidU{80 -- 120}
\def\aLIGOLate{140}
\def\aLIGOLateU{120 -- 170}
\def\aLIGOFinal{200}
\def\aLIGOFinalBNS{215}
\def\AdVInitial{20}
\def\AdVEarly{40}
\def\AdVEarlyU{20 -- 60}
\def\AdVMid{70}
\def\AdVMidU{60 -- 85}
\def\AdVLate{100}
\def\AdVLateU{65 -- 115}
\def\AdVFinal{130}
\def\AdVFinalBNS{145}

% journals
\providecommand{\jcap}[0]{JCAP}
\def\aj{Astronomical Journal}                 % Astronomical Journal
\def\apj{Astrophysical Journal}                % Astrophysical Journal
\def\apjl{Astrophysical Journal Letters}             % Astrophysical Journal, Letters
\def\pasj{PASJ}
\def\apjs{ApJS}              % Astrophysical Journal, Supplement
\def\mnras{MNRAS}            % Monthly Notices of the RAS
\def\prd{Physical Review D}       % Physical Review D
\def\prx{Physical Review X}       % Physical Review X
\def\prl{Physical Review Letters}    % Physical Review Letters
\def\cqg{Classical \& Quantum Gravity}%Classical and Quantum Gravity
\def\nat{Nature}              % Nature
\def\physrep{Physics Reports} % Physics Reports
\def\na{New Astronomy}		% New Astronomy
\def\aapr{Astronomy \& Astrophysics Reviews}	%Astronomy and Astrophysics Reviews
\def\araa{Annual Reviews of Astronomy \& Astrophysics} 
\def\aap{Astronomy \& Astrophysics}

% other
\newacronym{\APPEC}{APPEC}{Astro-Particle Physics European Consortium}
\newacronym{\ILC}{ILC}{International Linear Collider}
\newacronym{\FALC}{FALC}{Funding Agencies for Large Colliders}
\newacronym{\ICFA}{ICFA}{International Committee for Future Accelerators}
\newacronym{\TMT}{TMT}{Thirty Meter Telescope}


==> structureold.tex <==
%----------------------------------------------------------------------------------------
%	VARIOUS REQUIRED PACKAGES
%----------------------------------------------------------------------------------------
\usepackage[top=2.54cm,bottom=2.54cm,left=2.54cm,right=2.54cm,headsep=10pt,letterpaper]{geometry} % Page margins

%\usepackage[top=3cm,bottom=3cm,left=3.2cm,right=3.2cm,headsep=10pt,letterpaper]{geometry} % Page margins previous to 30.04.2019; then DMcC realised Science case team had changed theirs
\usepackage{xcolor} % Required for specifying colors by name
\definecolor{ocre}{RGB}{52,177,201} % Define the orange color used for highlighting throughout the book

% Font Settings
\usepackage{avant} % Use the Avantgarde font for headings
%\usepackage{times} % Use the Times font for headings
\usepackage{mathptmx} % Use the Adobe Times Roman as the default text font together with math symbols from the Sym­bol, Chancery and Computer Modern fonts

\usepackage{microtype} % Slightly tweak font spacing for aesthetics
\usepackage[utf8]{inputenc} % Required for including letters with accents
\usepackage[T1]{fontenc} % Use 8-bit encoding that has 256 glyphs

% Bibliography
%\usepackage[style=alphabetic,sorting=nyt,sortcites=true,autopunct=true,babel=hyphen,hyperref=true,abbreviate=false,backref=true,backend=biber]{biblatex}
%\addbibresource{bibliography.bib} % BibTeX bibliography file
%\defbibheading{bibempty}{}


\usepackage{titlesec} % Allows customization of titles

\usepackage{graphicx} % Required for including pictures
\graphicspath{{Pictures/}{figures/cosmo/}} % Specifies the directory where pictures are stored

\usepackage{lipsum} % Inserts dummy text

\usepackage{tikz} % Required for drawing custom shapes

\usepackage[english]{babel} % English language/hyphenation

\usepackage{enumitem} % Customize lists
\setlist{nolistsep} % Reduce spacing between bullet points and numbered lists

\usepackage{booktabs} % Required for nicer horizontal rules in tables

\usepackage{eso-pic} % Required for specifying an image background in the title page

%----------------------------------------------------------------------------------------
%	MAIN TABLE OF CONTENTS
%----------------------------------------------------------------------------------------

\usepackage{titletoc} % Required for manipulating the table of contents

\contentsmargin{0cm} % Removes the default margin
% Chapter text styling
\titlecontents{chapter}[1.25cm] % Indentation
{\addvspace{15pt}\large\sffamily\bfseries} % Spacing and font options for chapters
{\color{ocre!60}\contentslabel[\Large\thecontentslabel]{1.25cm}\color{ocre}} % Chapter number
{}
{\color{ocre!60}\normalsize\sffamily\bfseries\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number
% Section text styling
\titlecontents{section}[1.25cm] % Indentation
{\addvspace{5pt}\sffamily\bfseries} % Spacing and font options for sections
{\contentslabel[\thecontentslabel]{1.25cm}} % Section number
{}
{\sffamily\hfill\color{black}\thecontentspage} % Page number
[]
% Subsection text styling
\titlecontents{subsection}[1.25cm] % Indentation
{\addvspace{1pt}\sffamily\small} % Spacing and font options for subsections
{\contentslabel[\thecontentslabel]{1.25cm}} % Subsection number
{}
{\sffamily\;\titlerule*[.5pc]{.}\;\thecontentspage} % Page number
[]

%----------------------------------------------------------------------------------------
%	MINI TABLE OF CONTENTS IN CHAPTER HEADS
%----------------------------------------------------------------------------------------

% Section text styling
\titlecontents{lsection}[0em] % Indendating
{\footnotesize\sffamily} % Font settings
{}
{}
{}

% Subsection text styling
\titlecontents{lsubsection}[.5em] % Indentation
{\normalfont\footnotesize\sffamily} % Font settings
{}
{}
{}

%----------------------------------------------------------------------------------------
%	PAGE HEADERS
%----------------------------------------------------------------------------------------

\usepackage{fancyhdr} % Required for header and footer configuration

\pagestyle{fancy}
\renewcommand{\chaptermark}[1]{\markboth{\sffamily\normalsize\bfseries\chaptername\ \thechapter.\ #1}{}} % Chapter text font settings
\renewcommand{\sectionmark}[1]{\markright{\sffamily\normalsize\thesection\hspace{5pt}#1}{}} % Section text font settings
\fancyhf{} \fancyhead[LE,RO]{\sffamily\normalsize\thepage} % Font setting for the page number in the header
\fancyhead[LO]{\rightmark} % Print the nearest section name on the left side of odd pages
\fancyhead[RE]{\leftmark} % Print the current chapter name on the right side of even pages
\renewcommand{\headrulewidth}{0.5pt} % Width of the rule under the header
\addtolength{\headheight}{2.5pt} % Increase the spacing around the header slightly
\renewcommand{\footrulewidth}{0pt} % Removes the rule in the footer
\fancypagestyle{plain}{\fancyhead{}\renewcommand{\headrulewidth}{0pt}} % Style for when a plain pagestyle is specified

% Removes the header from odd empty pages at the end of chapters
\makeatletter
\renewcommand{\cleardoublepage}{
\clearpage\ifodd\c@page\else
\hbox{}
\vspace*{\fill}
\thispagestyle{empty}
%\newpage
\fi}

%----------------------------------------------------------------------------------------
%	THEOREM STYLES
%----------------------------------------------------------------------------------------

\usepackage{amsmath,amsfonts,amssymb,amsthm} % For math equations, theorems, symbols, etc

\newcommand{\intoo}[2]{\mathopen{]}#1\,;#2\mathclose{[}}
\newcommand{\ud}{\mathop{\mathrm{{}d}}\mathopen{}}
\newcommand{\intff}[2]{\mathopen{[}#1\,;#2\mathclose{]}}
\newtheorem{notation}{Notation}[chapter]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% dedicated to boxed/framed environements %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheoremstyle{ocrenumbox}% % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% % Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% % Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\renewcommand{\qedsymbol}{$\blacksquare$}% Optional qed square

\newtheoremstyle{blacknumex}% Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% Body font
{} % Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily{\tiny\ensuremath{\blacksquare}}\nobreakspace\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

\newtheoremstyle{blacknumbox} % Theorem style name
{0pt}% Space above
{0pt}% Space below
{\normalfont}% Body font
{}% Indent amount
{\small\bf\sffamily}% Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries---\nobreakspace#3.}}% Optional theorem note

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% dedicated to non-boxed/non-framed environements %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheoremstyle{ocrenum}% % Theorem style name
{5pt}% Space above
{5pt}% Space below
{\normalfont}% % Body font
{}% Indent amount
{\small\bf\sffamily\color{ocre}}% % Theorem head font
{\;}% Punctuation after theorem head
{0.25em}% Space after theorem head
{\small\sffamily\color{ocre}\thmname{#1}\nobreakspace\thmnumber{\@ifnotempty{#1}{}\@upn{#2}}% Theorem text (e.g. Theorem 2.1)
\thmnote{\nobreakspace\the\thm@notefont\sffamily\bfseries\color{black}---\nobreakspace#3.}} % Optional theorem note
\renewcommand{\qedsymbol}{$\blacksquare$}% Optional qed square
\makeatother

% Defines the theorem text style for each type of theorem to one of the three styles above
\newcounter{dummy}
\numberwithin{dummy}{section}
\theoremstyle{ocrenumbox}
\newtheorem{theoremeT}[dummy]{Theorem}
\newtheorem{problem}{Problem}[chapter]
\newtheorem{exerciseT}{Exercise}[chapter]
\theoremstyle{blacknumex}
\newtheorem{exampleT}{Example}[chapter]
\theoremstyle{blacknumbox}
\newtheorem{vocabulary}{Vocabulary}[chapter]
\newtheorem{definitionT}{Definition}[section]
\newtheorem{corollaryT}[dummy]{Corollary}
\theoremstyle{ocrenum}
\newtheorem{proposition}[dummy]{Proposition}

%----------------------------------------------------------------------------------------
%	DEFINITION OF COLORED BOXES
%----------------------------------------------------------------------------------------

\RequirePackage[framemethod=default]{mdframed} % Required for creating the theorem, definition, exercise and corollary boxes

% Theorem box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
backgroundcolor=black!5,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
innerbottommargin=5pt]{tBox}

% Exercise box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
backgroundcolor=ocre!10,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
innerbottommargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt]{eBox}

% Definition box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=ocre,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=0pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=0pt]{dBox}

% Corollary box
\newmdenv[skipabove=7pt,
skipbelow=7pt,
rightline=false,
leftline=true,
topline=false,
bottomline=false,
linecolor=gray,
backgroundcolor=black!5,
innerleftmargin=5pt,
innerrightmargin=5pt,
innertopmargin=5pt,
leftmargin=0cm,
rightmargin=0cm,
linewidth=4pt,
innerbottommargin=5pt]{cBox}

% Creates an environment for each type of theorem and assigns it a theorem text style from the "Theorem Styles" section above and a colored box from above
\newenvironment{theorem}{\begin{tBox}\begin{theoremeT}}{\end{theoremeT}\end{tBox}}
\newenvironment{exercise}{\begin{eBox}\begin{exerciseT}}{\hfill{\color{ocre}\tiny\ensuremath{\blacksquare}}\end{exerciseT}\end{eBox}}
\newenvironment{definition}{\begin{dBox}\begin{definitionT}}{\end{definitionT}\end{dBox}}
\newenvironment{example}{\begin{exampleT}}{\hfill{\tiny\ensuremath{\blacksquare}}\end{exampleT}}
\newenvironment{corollary}{\begin{cBox}\begin{corollaryT}}{\end{corollaryT}\end{cBox}}

%----------------------------------------------------------------------------------------
%	REMARK ENVIRONMENT
%----------------------------------------------------------------------------------------

\newenvironment{remark}{\par\vspace{10pt}\small % Vertical white space above the remark and smaller font size
\begin{list}{}{
\leftmargin=35pt % Indentation on the left
\rightmargin=25pt}\item\ignorespaces % Indentation on the right
\makebox[-2.5pt]{\begin{tikzpicture}[overlay]
\node[draw=ocre!60,line width=1pt,circle,fill=ocre!25,font=\sffamily\bfseries,inner sep=2pt,outer sep=0pt] at (-15pt,0pt){\textcolor{ocre}{R}};\end{tikzpicture}} % Orange R in a circle
\advance\baselineskip -1pt}{\end{list}\vskip5pt} % Tighter line spacing and white space after remark

%----------------------------------------------------------------------------------------
%	SECTION NUMBERING IN THE MARGIN

%----------------------------------------------------------------------------------------\titlespacing*{<command>}{<left>}{<before-sep>}{<after-sep>}

\makeatletter
\renewcommand{\@seccntformat}[1]{\llap{\textcolor{ocre}{\csname the#1\endcsname}\hspace{1em}}}
\renewcommand{\section}{\@startsection{section}{1}{\z@}
{-2ex \@plus -1ex \@minus -.4ex}
{1ex \@plus.2ex }
{\normalfont\large\sffamily\bfseries}}
\renewcommand{\subsection}{\@startsection {subsection}{2}{\z@}
{-1ex \@plus -0.1ex \@minus -.4ex}
{0.5ex \@plus.2ex }
{\normalfont\sffamily\bfseries}}
\renewcommand{\subsubsection}{\@startsection {subsubsection}{3}{\z@}
{-1ex \@plus -0.1ex \@minus -.2ex}
{.2ex \@plus.2ex }
{\normalfont\small\sffamily\bfseries}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}
{-1ex \@plus-.2ex \@minus .2ex}
{.1ex}
{\normalfont\small\sffamily\bfseries}}

%----------------------------------------------------------------------------------------
%	HYPERLINKS IN THE DOCUMENTS
%----------------------------------------------------------------------------------------

% For an unclear reason, the package should be loaded now and not later
\usepackage[colorlinks=true,citecolor=blue,linkcolor=blue]{hyperref}
%\hypersetup{hidelinks,backref=true,pagebackref=true,hyperindex=true,colorlinks=false,breaklinks=true,urlcolor= ocre,bookmarks=true,bookmarksopen=false,pdftitle={Title},pdfauthor={Author}}

%----------------------------------------------------------------------------------------
%	CHAPTER HEADINGS
%----------------------------------------------------------------------------------------

% The set-up below should be (sadly) manually adapted to the overall margin page septup controlled by the geometry package loaded in the main.tex document. It is possible to implement below the dimensions used in the goemetry package (top,bottom,left,right)... TO BE DONE

\newcommand{\thechapterimage}{}
\newcommand{\chapterimage}[1]{\renewcommand{\thechapterimage}{#1}}

% Numbered chapters with mini tableofcontents
\def\thechapter{\arabic{chapter}}
\def\@makechapterhead#1{
\thispagestyle{empty}
{\centering \normalfont\sffamily
\ifnum \c@secnumdepth >\m@ne
\if@mainmatter
\startcontents
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\includegraphics[width=\paperwidth]{\thechapterimage}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commenting the 3 lines below removes the small contents box in the chapter heading
%\fill[color=ocre!10!white,opacity=.6] (1cm,0) rectangle (8cm,-7cm);
%\node[anchor=north west] at (1.1cm,.35cm) {\parbox[t][8cm][t]{6.5cm}{\huge\bfseries\flushleft \printcontents{l}{1}{\setcounter{tocdepth}{2}}}};
\draw[anchor=west] (2cm,-9cm) node [rounded corners=20pt,fill=ocre!10!white,text opacity=1,draw=ocre,draw opacity=1,line width=1.5pt,fill opacity=.6,inner sep=12pt]{\huge\sffamily\bfseries\textcolor{black}{\thechapter. #1\strut\makebox[22cm]{}}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tikzpicture}};
\end{tikzpicture}}
\par\vspace*{230\p@}
\fi
\fi}

% Unnumbered chapters without mini tableofcontents (could be added though)
\def\@makeschapterhead#1{
\thispagestyle{empty}
{\centering \normalfont\sffamily
\ifnum \c@secnumdepth >\m@ne
\if@mainmatter
\begin{tikzpicture}[remember picture,overlay]
\node at (current page.north west)
{\begin{tikzpicture}[remember picture,overlay]
\node[anchor=north west,inner sep=0pt] at (0,0) {\includegraphics[width=\paperwidth]{\thechapterimage}};
\draw[anchor=west] (10cm,-9cm) node [rounded corners=20pt,fill=ocre!10!white,fill opacity=.6,inner sep=12pt,text opacity=1,draw=ocre,draw opacity=1,line width=1.5pt]{\huge\sffamily\bfseries\textcolor{black}{#1\strut\makebox[22cm]{}}};
\end{tikzpicture}};
\end{tikzpicture}}
\par\vspace*{230\p@}
\fi
\fi
}
\makeatother


%needed for cosmo
\usepackage{graphicx}
\graphicspath{{./figures/}}
%\usepackage{psfrag}
\usepackage{appendix}
\usepackage{latexsym,amsmath,amsfonts,amssymb,booktabs}
\usepackage[font=small]{caption}
\usepackage{slashed,upgreek,amscd,cancel,tensor,color}
\usepackage{adjustbox}
\usepackage[numbers,compress,square]{natbib}
\usepackage{epsfig,latexsym}
%\usepackage[pdfencoding=auto]{hyperref}
\usepackage{url}
\numberwithin{equation}{section}% numera le equazioni seconde le sezioni , e.g. 1.15 invece che consecutivamente; anche le appendici, eq. (A.1) etc. Richiede amsmath
\usepackage{doi}
\usepackage{subcaption}
\usepackage{mathtools}
\usepackage{textcomp}
\usepackage{upgreek}
\usepackage{stfloats}
\usepackage{afterpage}
\usepackage{multirow}

%\newcommand{\mnras}{MNRAS}
%\newcommand{\aap}{A\&A}
%\newcommand{\nat}{Nature}
%\newcommand{\araa}{Annual Review of Astronomy and Astrophysics}
%\newcommand{\araa}{ARAA}
%\newcommand{\apj}{ApJ}
%\newcommand{\apjl}{ApJL}
%\newcommand{\aj}{AJ}
%\newcommand{\prd}{Physical Reviews D}
\newcommand{\aapr}{Astronomy and Astrophysics Reviews}

\definecolor{antiquewhite}{rgb}{0.98, 0.92, 0.84}
\definecolor{aliceblue}{rgb}{0.94, 0.97, 1.0}
\definecolor{blanchedalmond}{rgb}{1.0, 0.92, 0.8}
\definecolor{beaublue}{rgb}{0.74, 0.83, 0.9}
\definecolor{beaubluedark}{rgb}{0.79, 0.85, 0.95}
\definecolor{amber(sae/ece)}{rgb}{1.0, 0.49, 0.0}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{aliceblue}{rgb}{0.94, 0.97, 1.0}
\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\definecolor{almond}{rgb}{0.94, 0.87, 0.8}
\definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
\definecolor{amber}{rgb}{1.0, 0.75, 0.0}
\definecolor{amber(sae/ece)}{rgb}{1.0, 0.49, 0.0}
\definecolor{americanrose}{rgb}{1.0, 0.01, 0.24}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{anti-flashwhite}{rgb}{0.95, 0.95, 0.96}
\definecolor{antiquebrass}{rgb}{0.8, 0.58, 0.46}
\definecolor{antiquefuchsia}{rgb}{0.57, 0.36, 0.51}
\definecolor{antiquewhite}{rgb}{0.98, 0.92, 0.84}
\definecolor{ao}{rgb}{0.0, 0.0, 1.0}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{apricot}{rgb}{0.98, 0.81, 0.69}
\definecolor{aqua}{rgb}{0.0, 1.0, 1.0}
\definecolor{aquamarine}{rgb}{0.5, 1.0, 0.83}
\definecolor{beaver}{rgb}{0.62, 0.51, 0.44}
\definecolor{blizzardblue}{rgb}{0.67, 0.9, 0.93}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}

\usepackage{pdfpages}
\usepackage[squaren]{SIunits}
\usepackage{acronym}
\usepackage{etoolbox}
\usepackage{multicol}
 \usepackage{vwcol}
\usepackage{placeins}
\usepackage[absolute]{textpos}
\usepackage{ulem} \normalem
\usepackage{tcolorbox}
\usepackage{wrapfig}
\newcommand{\redcomment}[1]{{\noindent\color{red}{\it [[#1]] }}}
\newcommand{\bluecomment}[1]{{\color{blue}{\it[[#1]]}}}
\newcommand{\magentacomment}[1]{{\color{magenta}{[[ #1]]}}}
\newcommand{\greencomment}[1]{{\color{green}{[[ #1]]}}}
\newcommand{\redtext}[1]{{\noindent\color{red}{\it #1 }}}

\newtcolorbox{DetBox}[2][]{%
standard jigsaw,colframe=green!40!black,colback=blanchedalmond!10!white,opacityback=0.6,coltext=black,oversize, size=small, title=Infobox~\theboxcount: #2,#1}

\newtcolorbox{Infobox}[2][]{%
standard jigsaw,colframe=ocre,colback=blanchedalmond!10!white,opacityback=0.6,coltext=black, size=small, title=Infobox~\theboxcount: #2,#1}

%\newcounter{myboxcount}
%\setcounter{myboxcount}{1}
\newcommand{\ao}{Applied Optics} 

==> unassigned_RaD_items.tex <==
%\chapterimage{Figures/balance.jpg} % Chapter heading image
% https://upload.wikimedia.org/wikipedia/commons/2/27/Bascula_9.jpg
\chapterimage{Figures/urmeter.jpg} % Chapter heading image
%https://www.lichtmikroskop.net/elektronenmikroskop/bilder/urmeter.jpg
\chapter{Calibration}
%\section{R\&D misc.}
\label{sec:Calibration}
%\section{Schumann resonances}
%Schumann resonances, global electromagnetic resonances propagating around the earth in the wave-guide formed by the earth and the ionosphere and excited by lightning discharges, can generate a correlated background in widely spaced gravitational wave detectors, which complicates the detection of a stochastic gravitational wave background. Dedicated detectors and models for the excitation and propagation of magnetic waves can be used to subtract the contributions from the gravitational wave signal. 

%Contacts (James Lough <james.lough@aei.mpg.de>, Yuki Inoue <iyuki@ncu.edu.tw>)
Extracting new science from the observed GWs requires accurate knowledge of the amplitude and timing of the signals. With high SNR detections expected in 3G detectors on the order of 1000, extremely low calibration uncertainty will be necessary for observations to be noise limited.

\section{Science driven calibration requirements}
%While the exact calibration requirements for the science we wish to do with 3G detectors is not well known, we can make some estimates. One might make the assumption that one would need something like 1/snr calibration accuracy, it's more complicated than this. The calibration uncertainty is frequency dependent. At some frequencies we don't know the calibration as well as other frequencies. At the same time, the signals we wish to analyze are frequency dependent. There are investigations underway to understand calibration requirements in a way that takes into account the signal, and the detector to determine required frequency dependent calibration uncertainty. With a detector network of 1 Einstein Telescope and 2 Cosmic Explorer detectors, we expect to see about 1 event per year of ~1000 SNR. At the highest SNRs, we can set the best limits on GR. To not be dominated by calibration error, we need to have calibration to within 0.5\% in amplitude.

The exact calibration requirements needed for the scientific objectives of 3G GW observatories are not yet known, but can be estimated. The calibration accuracy not only depends on the SNR of the signal, but both the detector calibration and the signal calibration are also frequency dependent. Studies are currently underway that take both aspects into account and evaluate the frequency response requirements of the calibration uncertainty.  With a detector network of three 3G detectors we expect about one event per year with SNR ~1000. The signals with the highest SNRs give the narrowest limits for GR. To avoid being dominated by calibration errors, we need a calibration \magentacomment{absolute or relative?} to an amplitude of 0.5\%.

The science we can do with detections in third generation detectors that will be limited by calibration include BNS tidal deformation, deviations from GR, and measurements of the Hubble constant. The first two look for deviations from a modeled waveform template, while the latter is based on absolute distance measurements.

There are two aspects of calibration uncertainty, the absolute uncertainty and the relative uncertainty. The first tells us how well we understand the total calibration in absolute numbers, while the latter is a frequency-dependent calibration uncertainty with respect to some fixed reference frequency. We have to consider each individually, depending on the physics we want to study. Looking for deviations from a modeled waveform template, we are mainly concerned with relative calibration uncertainty. In order to understand the absolute distance to the sources, we are most interested in absolute calibration.

\section{State of the art in calibration}
\subsection{Photon calibrators}
Photon calibrators (PCAL) provide a calibration reference starting from a traceable reference power meter. They use an amplitude modulated laser to apply a photon-recoil force to the test mass. For all large scale interferometric Gravitational Wave Detectors this is the current method of choice for absolute calibration. 
PCAL reference uncertainty is roughly at the 1\% level. This was specifically stated at 0.76\% for the O2 calibration uncertainty for the advanced LIGO detectors.\magentacomment{citation needed} This resulted in a frequency dependent uncertainty between 2\% and 4\% for O2\magentacomment{How does an absolute calibration uncertainty of 0.76\% result in a relative uncertainty of 2\% - 4\%? ,citation needed}. With improvements between O2 and O3 the expectation is that this could be reduced to \magentacomment{a relative uncertainty? of} 0.3\%.\magentacomment{citation needed.} 

\subsection{Newtonian calibrators}
This calibration method relies on gravitational interaction between an arrangement of rapidly rotating assymetrically arranged masses and one of the interferometer test masses. Adding a gravity field calibrator to the photon calibrator results in a theoretical absolute calibration uncertainty of 0.17\% .\cite{PhysRevD.98.022005}
advanced LIGO, advanced Virgo, and KAGRA are all developing Newtonian calibrator technologies.\cite{PhysRevD.98.022005,0264-9381-35-23-235009}

The design for the {\bf KAGRA} gravity field calibrator incorporates two distinct mass distributions in one rotating mass. One quadrupole and one hexapole, which provide a sort of self calibration of the distance to the test mass.\cite{PhysRevD.98.022005}\par
{\bf Advanced LIGO} is also working on a Newtonian calibrator for confirmation of the photon calibrator in a similar way to KAGRA.\magentacomment{citation needed} \par
{\bf Advanced Virgo} has recently published \cite{0264-9381-35-23-235009}  first tests of such a system and observed less than 1\% statistical uncertainty at some frequencies.\par
These Newtonian calibrator technologies are still in the very early stages of development, but there is significant work effort in this direction.

\subsection{Frequency based calibration}
Another calibration method would be to use frequencies as a reference. We can measure frequencies much more precisely than amplitudes. Free swinging Michelson is an example of this technique, though with arm cavities this method has to be done in steps and involves actuating the ITMs through the PUM stage which is weak and introduces more error than what is achievable with PCAL. For detectors without arm cavities (such as GEO 600) this method is much simpler and can result in very precise measurements of the absolute ESD actuator calibration, with statistical uncertainties of less than 0.1\%. \cite{Leong2012}

The arm cavity locking method outlined in the LIGO calibration for GW150914 paper is another example.
\cite{PhysRevD.95.062003}
This uses a frequency reference which in this case would be an RF LO to measure the beat frequency between the green arm locking signal and the frequency doubled infrared light.


